Natural Language Rationales with Full-Stack Visual Reasoning: From Pixels to Semantic Frames to Commonsense Graphs

Natural language rationales could provide intuitive, higher-level explanations that are easily understandable by humans, complementing the more broadly studied lower-level explanations based on gradients or attention weights. We present the first study focused on generating natural language rationales across several complex visual reasoning tasks: visual commonsense reasoning, visual-textual entailment, and visual question answering. The key challenge of accurate rationalization is comprehensive image understanding at all levels: not just their explicit content at the pixel level, but their contextual contents at the semantic and pragmatic levels. We present Rationale^VT Transformer, an integrated model that learns to generate free-text rationales by combining pretrained language models with object recognition, grounded visual semantic frames, and visual commonsense graphs. Our experiments show that the base pretrained language model benefits from visual adaptation and that free-text rationalization is a promising research direction to complement model interpretability for complex visual-textual reasoning tasks.

==> tables/4_e_snli_ve_multimodal_plausibility_breakdown.tex <==
\begin{table}[!ht]
\resizebox{\columnwidth}{!}{
\begin{tabular}{l@{\hskip 2mm}l@{\hskip 4mm}l@{\hskip 4mm}lcc}
\toprule
&&&&\multicolumn{2}{c}{\textbf{\esnlive}}\\
\cmidrule{5-6}
 &&   &   & contradiction & entailment \\
    \midrule
&&  & Baseline   & 46.85  {\small($\downarrow$27.63)}             & \textbf{46.76}      {\small($\uparrow$ 0.48)}            \\
  \midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{Rationale}$^{\textsc{VT}}$}} & \multirow{6}{*}{\rotatebox{90}{\textsc{Transformers}}}&\multirow{3}{*}{\rotatebox{90}{\small\uniform}} & Object labels       & 58.56   {\small($\downarrow$ 18.92)}              & 36.45  {\small($\downarrow$0.72)}                \\
  &&  & Situation frame            & 59.16  {\small($\downarrow$ 13.21)}              & 38.13        {\small($\downarrow$ 0.48)}          \\
 &&   & \viscomet  text         & 53.75   {\small($\downarrow$ 17.42)}             & 29.26       {\small($\downarrow$3.12)}           \\
\cmidrule{3-6}
&&\multirow{3}{*}{\rotatebox{90}{\small\hybrid}} & Object regions          & \textbf{60.96}              {\small($\downarrow$ 9.01)}  & 34.05 {\small($\uparrow$0.24)}                 \\
&&                         & Situ.\ Roles regions & 51.95  {\small($\downarrow$ 10.51)}              & 37.65       {\small($\downarrow$0.96)}           \\
&&                         & \viscomet embed.\              & 48.95 {\small($\downarrow$ 25.83)}                & 32.13         {\small($\downarrow$ 0.24)}   \\  
\midrule
\midrule
&&& Human (estimate) & 80.78 {\small($\uparrow$ 1.20)} & 76.98       {\small($\uparrow$2.64)}           \\
\bottomrule
\end{tabular}
}
\caption{Breakdown of \textit{visual} plausibility for \esnlive with respect to the entailment label. Our baseline is text-only \gpt. The best model is boldfaced.}
\label{tab:multimodal_plausibility_e_snli_ve_breakdown}
\end{table}






==> tables/4_generation_examples.tex <==
\begin{table*}[!ht]
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{ll}
  \toprule
    \begin{minipage}{6cm}
      \includegraphics[width=6cm]{tables/4_example_vcr_generation.png}
    \end{minipage}
    &
    \begin{tabular}{m{10cm}}
        \textbf{Question:} What would happen if [person5] stood up? \\[0.2cm]
        \textbf{Answer:} [person5] would knock over [diningtable1]. \\[0.2cm]
        \textbf{Generated Rationale:} [person5] is sitting at diningtable and diningtable is directly in front of her. \\[0.5cm]
        \textbf{Gold Rationale}: [person5] is sitting underneath [diningtable1].
    \end{tabular}\\
            \midrule
        \begin{minipage}{6cm}
      \includegraphics[width=6cm]{tables/4_example_esnli_generation.jpg}
    \end{minipage}
    &
    \begin{tabular}{m{10cm}}
        \textbf{Hypothesis:} A woman is texting. \\[0.2cm]
        \textbf{Label:} contradiction \\[0.2cm]
        \textbf{Generated Rationale:} A woman can not be texting while she is talking on a cellphone. \\[0.5cm]
        \textbf{Gold Rationale}: The person is either texting or talking.
    \end{tabular}\\
    \midrule
        \begin{minipage}{6cm}
      \includegraphics[width=6cm]{tables/4_example_vqa_generation.jpg}
    \end{minipage}
    &
    \begin{tabular}{m{10cm}}
        \textbf{Question:} Is the train on a track? \\[0.2cm]
        \textbf{Answer:} yes \\[0.2cm]
        \textbf{Generated Rationale:} People are waiting at a train station for the train to stop. \\[0.5cm]
        \textbf{Gold Rationale:} A train at the station surrounded by people.
    \end{tabular}\\
  \bottomrule
  \end{tabular}
  }
  \caption{\modelname generations for \vcr, \esnlive (contradiction), and \vqae, respectively. We use the best model variant for each dataset (according to results in Tables \ref{tab:results_plausibility_with_image}--\ref{tab:multimodal_plausibility_e_snli_ve_breakdown}).}
  \label{tab:generation_examples}
\end{table*}
